An Online Learning Approach to Shortest Path and Backpressure Routing in Wireless Networks

We consider the adaptive routing problem in multihop wireless networks. The link states are assumed to be random variables drawn from unknown distributions, independent and identically distributed across links and time. This model has attracted a growing interest recently in cognitive radio networks and adaptive communication systems. In such networks, devices are cognitive in the sense of learning the link states and updating the transmission parameters to allow efficient resource utilization. This model contrasts sharply with the vast literature on routing algorithms that assumed complete knowledge about the link state means. The goal is to design an algorithm that learns online optimal paths for data transmissions to maximize the network throughput while attaining low path cost over flows in the network. We develop a novel Online Learning for Shortest path and Backpressure (OLSB) algorithm to achieve this goal. We analyze the performance of OLSB rigorously and show that it achieves a logarithmic regret with time, defined as the loss of an algorithm as compared to a genie that has complete knowledge about the link state means. We further evaluate the performance of OLSB numerically via extensive simulations, which support the theoretical findings and demonstrate its high efficiency.

==> macros.tex <==

%%%%%%%%%%%%%5
% new symbols
%\newcommand{\force}{\mbox{$\parallel \! \! \! -$}}
\newcommand{\force}{\mbox{$\Vdash$}}

% Hatted english letters
\newcommand{\ghat}{\mbox{$\bm \hat g$}}

\newcommand{\bzero}{\mbox{${\bm 0}$}}

% abbreviations for bold english letters (vectors)
\newcommand{\va}{\mbox{${\mathbf a}$}}
\newcommand{\vah}{\mbox{${\mathbf \hat a}$}}
\newcommand{\vat}{\mbox{${\mathbf \tilde a}$}}
\newcommand{\vb}{\mbox{${\mathbf b}$}}
\newcommand{\vd}{\mbox{${\mathbf d}$}}
\newcommand{\rh}{\mbox{${\hat r}$}}


\newcommand{\vxt}{\mbox{${\mathbf \tilde x}$}}
\newcommand{\vh}{\mbox{${\mathbf h}$}}
\newcommand{\vhh}{\mbox{${\mathbf \hat h}$}}
\newcommand{\ve}{\mbox{${\mathbf e}$}}
\newcommand{\vg}{\mbox{${\mathbf g}$}}
\newcommand{\vgh}{\mbox{${\mathbf \hat g}$}}
\newcommand{\vp}{\mbox{${\mathbf p}$}}
\newcommand{\vq}{\mbox{${\mathbf q}$}}
\newcommand{\vt}{\mbox{${\mathbf t}$}}
\newcommand{\vw}{\mbox{${\mathbf w}$}}
\newcommand{\vwh}{\mbox{${\mathbf \hat w}$}}
\newcommand{\wh}{\mbox{${\hat w}$}}
\newcommand{\vwt}{\mbox{${\mathbf \tilde w}$}}
\newcommand{\wt}{\mbox{${\tilde w}$}}
\newcommand{\vs}{\mbox{${\mathbf s}$}}
\newcommand{\vsh}{\mbox{${\mathbf \hat s}$}}
\newcommand{\vst}{\mbox{${\mathbf \tilde s}$}}
\newcommand{\vr}{\mbox{${\mathbf r}$}}
\newcommand{\vx}{\mbox{${\mathbf x}$}}
\newcommand{\vv}{\mbox{${\mathbf v}$}}
\newcommand{\vu}{\mbox{${\mathbf u}$}}
\newcommand{\vy}{\mbox{${\mathbf y}$}}
\newcommand{\vz}{\mbox{${\mathbf z}$}}
\newcommand{\vn}{\mbox{${\mathbf n}$}}
\newcommand{\vnt}{\mbox{${\mathbf \tilde n}$}}
\newcommand{\vzero}{\mbox{${\mathbf 0}$}}
\newcommand{\vone}{\mbox{${\mathbf 1}$}}

% abbreviations for matrices
\newcommand{\mA}{\mbox{{$\mathbf A$}}}
\newcommand{\mAh}{\mbox{${\mathbf \hat A}$}}
\newcommand{\mAt}{\mbox{$\mathbf \tilde A$}}
\newcommand{\mB}{\mbox{${\mathbf B}$}}
\newcommand{\mBh}{\mbox{${\mathbf \hat B}$}}
\newcommand{\mC}{\mbox{{$\mathbf C$}}}
\newcommand{\mCh}{\mbox{${\mathbf \hat C}$}}
\newcommand{\mD}{\mbox{{$\mathbf D$}}}
\newcommand{\mDt}{\mbox{$\mathbf \tilde D$}}
\newcommand{\mE}{\mbox{{$\mathbf E$}}}
\newcommand{\mG}{\mbox{{$\mathbf G$}}}
\newcommand{\mF}{\mbox{{$\mathbf F$}}}
\newcommand{\mH}{\mbox{{$\mathbf H$}}}
\newcommand{\mHb}{\mbox{${\mathbf \bar H}$}}
\newcommand{\mI}{\mbox{{$\mathbf I$}}}
\newcommand{\mIh}{\mbox{${\mathbf \hat I}$}}
\newcommand{\mN}{\mbox{{$\mathbf N$}}}
\newcommand{\mM}{\mbox{{$\mathbf M$}}}
\newcommand{\mMh}{\mbox{{$\mathbf \hat M$}}}
\newcommand{\mP}{\mbox{${\mathbf P}$}}
\newcommand{\mQ}{\mbox{${\mathbf Q}$}}
\newcommand{\mR}{\mbox{${\mathbf R}$}}
\newcommand{\mRh}{\mbox{${\mathbf {\hat {R}}}$}}
\newcommand{\mRt}{\mbox{${\mathbf \tilde R}$}}
\newcommand{\mS}{\mbox{${\mathbf S}$}}
\newcommand{\mSb}{\mbox{${\mathbf \bar S}$}}
\newcommand{\mSh}{\mbox{${\mathbf \hat S}$}}
\newcommand{\mSt}{\mbox{${\mathbf \tilde S}$}}
\newcommand{\mT}{\mbox{${\mathbf T}$}}
\newcommand{\mU}{\mbox{${\mathbf U}$}}
\newcommand{\mUh}{\mbox{${\mathbf \hat U}$}}
\newcommand{\mV}{\mbox{${\mathbf V}$}}
\newcommand{\mVh}{\mbox{${\mathbf \hat V}$}}
\newcommand{\mW}{\mbox{${\mathbf W}$}}
\newcommand{\mWh}{\mbox{${\mathbf \hat W}$}}
\newcommand{\mWt}{\mbox{${\mathbf \tilde W}$}}
\newcommand{\mX}{\mbox{${\mathbf X}$}}
\newcommand{\mY}{\mbox{${\mathbf Y}$}}
\newcommand{\mZ}{\mbox{${\mathbf Z}$}}



%abbreviations for greek letters

\newcommand{\ga}{\alpha}
\newcommand{\gb}{\beta}
\newcommand{\grg}{\gamma}
\newcommand{\gd}{\delta}
\newcommand{\gre}{\varepsilon}
\newcommand{\gep}{\epsilon}
\newcommand{\gz}{\zeta}
\newcommand{\gzh}{\mbox{$ \hat \zeta$}}
\newcommand{\gh}{\eta}
\newcommand{\gth}{\theta}
\newcommand{\gi}{iota}
\newcommand{\gk}{\kappa}
\newcommand{\gl}{\lambda}
\newcommand{\gm}{\mu}
\newcommand{\gn}{\nu}
\newcommand{\gx}{\xi}
\newcommand{\gp}{\pi}
\newcommand{\gph}{\phi}
\newcommand{\gr}{\rho}
\newcommand{\gs}{\sigma}
\newcommand{\gsh}{\hat \sigma}
\newcommand{\gt}{\tau}
\newcommand{\gu}{\upsilon}
\newcommand{\gf}{\varphi}
\newcommand{\gc}{\chi}
\newcommand{\go}{\omega}

%Uppercase Greek

\newcommand{\gG}{\Gamma}
\newcommand{\gD}{\Delta}
\newcommand{\gTh}{\Theta}
\newcommand{\gL}{\Lambda}
\newcommand{\gX}{\Xi}
\newcommand{\gP}{\Pi}
\newcommand{\gS}{\Sigma}
\newcommand{\gU}{\Upsilon}
\newcommand{\gF}{\Phi}
\newcommand{\gO}{\Omega}

%Uppercase bold Greek

\def\bm#1{\mbox{\boldmath $#1$}}
\newcommand{\vga}{\mbox{$\bm \alpha$}}
\newcommand{\vgb}{\mbox{$\bm \beta$}}
\newcommand{\vgd}{\mbox{$\bm \delta$}}
\newcommand{\vge}{\mbox{$\bm \epsilon$}}
\newcommand{\vgl}{\mbox{$\bm \lambda$}}
\newcommand{\vgr}{\mbox{$\bm \rho$}}
\newcommand{\vgrh}{\mbox{$\bm \hat \rho$}}
\newcommand{\vgrt}{\mbox{$\bm {\tilde \rho}$}}

\newcommand{\vgt}{\mbox{$\bm \gt$}}
\newcommand{\vgth}{\mbox{$\bm {\hat \tau}$}}
\newcommand{\vgtt}{\mbox{$\bm {\tilde \tau}$}}
\newcommand{\vpsi}{\mbox{$\bm \psi$}}
\newcommand{\vphi}{\mbox{$\bm \phi$}}
\newcommand{\vxi}{\mbox{$\bm \xi$}}
\newcommand{\vth}{\mbox{$\bm \theta$}}
\newcommand{\vthh}{\mbox{$\bm {\hat \theta}$}}

\newcommand{\mgG}{\mbox{$\bm \Gamma$}}
\newcommand{\mgGh}{\mbox{$\hat {\bm \Gamma}$}}
\newcommand{\mgD}{\mbox{$\bm \Delta$}}
\newcommand{\mgU}{\mbox{$\bm \Upsilon$}}
\newcommand{\mgL}{\mbox{$\bm \Lambda$}}
\newcommand{\mPsi}{\mbox{$\bm \Psi$}}
\newcommand{\mgX}{\mbox{$\bm \Xi$}}
\newcommand{\mgS}{\mbox{$\bm \Sigma$}}

%Abbreviatians for blackboard bold
\newcommand{\oA}{{\open A}}
\newcommand{\oC}{{\open C}}
\newcommand{\oF}{{\open F}}
\newcommand{\oN}{{\open N}}
\newcommand{\oP}{{\open P}}
\newcommand{\oQ}{{\open Q}}
\newcommand{\oR}{{\open R}}
\newcommand{\oZ}{{\open Z}}

%Abbreviatians for caligraphic letters

\newcommand{\Nu}{{\cal V}}
\newcommand{\cA}{{\cal A}}
\newcommand{\cB}{{\cal B}}
\newcommand{\cC}{{\cal C}}
\newcommand{\cD}{{\cal D}}
\newcommand{\cF}{{\cal F}}
\newcommand{\cH}{{\cal H}}
\newcommand{\cK}{{\cal K}}
\newcommand{\cI}{{\cal I}}
\newcommand{\cL}{{\cal L}}
\newcommand{\cM}{{\cal M}}
\newcommand{\cN}{{\cal N}}
\newcommand{\cO}{{\cal O}}
\newcommand{\cP}{{\cal P}}
\newcommand{\cR}{{\cal R}}
\newcommand{\cS}{{\cal S}}
\newcommand{\cU}{{\cal U}}
\newcommand{\cV}{{\cal V}}
\newcommand{\cT}{{\cal T}}
\newcommand{\cX}{{\cal X}}

%\newcommand{\rH}{^{ \raisebox{1pt}{$\rm \scriptscriptstyle H$}}}
\newcommand{\rH}{^{*}}
\newcommand{\rT}{^{ \raisebox{1.2pt}{$\rm \scriptstyle T$}}}
\newcommand{\rF}{_{ \raisebox{-1pt}{$\rm \scriptstyle F$}}}
\newcommand{\rE}{{\rm E}}

% mathematical functions and constants
\newcommand{\dom}{\hbox{dom}}
\newcommand{\rng}{\hbox{rng}}
\newcommand{\Span}{\hbox{span}}
\newcommand{\Ker}{\hbox{Ker}}
\newcommand{\On}{\hbox{On}}
\newcommand{\otp}{\hbox{otp}}
\newcommand{\ZFC}{\hbox{ZFC}}
\def\Re{\ensuremath{\hbox{Re}}}
\def\Im{\ensuremath{\hbox{Im}}}
\newcommand{\SNR}{\ensuremath{\hbox{SNR}}}
\newcommand{\SINR}{\ensuremath{\hbox{SINR}}}
\newcommand{\NI}{\ensuremath{\hbox{NI}}}
\newcommand{\CRB}{\ensuremath{\hbox{CRB}}}
\newcommand{\diag}{\ensuremath{\hbox{diag}}}
\newcommand{\trace}{\ensuremath{\hbox{tr}}}
\newcommand{\E}{\ensuremath{\hbox{\textbf{E}}}}
\newcommand{\DR}{\ensuremath{\hbox{DR}}}

% more complex mathematical entities
\newcommand{\dlot}{\mbox{$\delta^1_3$}}
\newcommand{\Dlot}{\mbox{$\Delta^1_3$}}
\newcommand{\Dlof}{\mbox{$\Delta^1_4$}}
\newcommand{\dlof}{\mbox{$\delta^1_4$}}
\newcommand{\bP}{\mbox{$\mathbf{P}$}}
\newcommand{\Pot}{\mbox{$\Pi^1_2$}}
\newcommand{\Sot}{\mbox{$\Sigma^1_2$}}
\newcommand{\gDot}{\mbox{$\gD^1_2$}}

\newcommand{\Potr}{\mbox{$\Pi^1_3$}}
\newcommand{\Sotr}{\mbox{$\Sigma^1_3$}}
\newcommand{\gDotr}{\mbox{$\gD^1_3$}}

\newcommand{\Pofr}{\mbox{$\Pi^1_4$}}
\newcommand{\Sofr}{\mbox{$\Sigma^1_4$}}
\newcommand{\Dofr}{\mbox{$\gD^1_4$}}


\newcommand{\Sa}{\mbox{$S_{\ga}$}}
\newcommand{\Qk}{\mbox{$Q_{\gk}$}}
\newcommand{\Ca}{\mbox{$C_{\ga}$}}

\newcommand{\gkp}{\mbox{$\gk^+$}}
\newcommand{\aron}{ Aronszajn }

\newcommand{\sqkp}{\mbox{$\Box_{\gk}$}}
\newcommand{\dkp}{\mbox{$\Diamond_{\gk^{+}}$}}
\newcommand{\sqsqnce}
{\mbox{\\ $\ < \Ca \mid \ga < \gkp \ \ \wedge \ \ \lim \ga >$ \ \ }}
\newcommand{\dsqnce}{\mbox{$<S_{\ga} \mid \ga < \gkp >$}}



%%%%%%%%%%%%%%%% Environnements %%%%%%%%%%%%%%%%%%
%\newcounter{theorem}
%\newtheorem{theorem}{Theorem}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{claim}[theorem]{Claim}
%\newcounter{definition}
%\newtheorem{definition}{Definition}
%
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{remark}{Remark}
\newtheorem{definition}{Definition}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}

%%%%%%%%%%%%%%%%%%% Preambule %%%%%%%%%%%%%%%%%%%%

% mathematical environments
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bea}{\begin{array}}
\newcommand{\ena}{\end{array}}
%\newcommand{\bds}{\begin {description}}
%\newcommand{\eds}{\end {description}}
\newcommand{\bds}{\begin {itemize}}
\newcommand{\eds}{\end {itemize}}
\newcommand{\bdf}{\begin{definition}}
\newcommand{\blm}{\begin{lemma}}
\newcommand{\edf}{\end{definition}}
\newcommand{\elm}{\end{lemma}}
\newcommand{\bthm}{\begin{theorem}}
\newcommand{\ethm}{\end{theorem}}
\newcommand{\bprp}{\begin{prop}}
\newcommand{\eprp}{\end{prop}}
\newcommand{\bcl}{\begin{claim}}
\newcommand{\ecl}{\end{claim}}
\newcommand{\bcr}{\begin{coro}}
\newcommand{\ecr}{\end{coro}}
\newcommand{\bquest}{\begin{question}}
\newcommand{\equest}{\end{question}}

%Abbreviatians for other symbols
\newcommand{\rarrow}{{\rightarrow}}
\newcommand{\Rarrow}{{\Rightarrow}}
\newcommand{\larrow}{{\larrow}}
\newcommand{\Larrow}{{\Leftarrow}}
\newcommand{\restrict}{{\upharpoonright}}
\newcommand{\nin}{{\not \in}}





%\newcommand{\ha}{\mbox{$\hat{\b{a}}$}}
%\newcommand{\tba}{\mbox{$\tilde{\b{a}}$}}
%\newcommand{\yh}{\mbox{${\hat y}$}}
%\newcommand{\vth}{\mbox{${\boldsymbol {\theta}}$}}
%\newcommand{\ups}{\mbox{${\Upsilon}$}}
%\newcommand{\vthh}{\mbox{${\boldsymbol {\hat \theta}}$}}
%\newcommand{\vtht}{\mbox{${\boldsymbol {\tilde \theta}}$}}
%\newcommand{\veps}{\mbox{${\underline \epsilon}$}}
%\newcommand{\vrho}{\mbox{${\boldsymbol {\rho}}$}}
%\newcommand{\vrhoh}{\mbox{${\boldsymbol {\hat \rho}}$}}
%\newcommand{\vrhot}{\mbox{${\boldsymbol {\tilde \rho}}$}}

%\newcommand{\vy}{\mbox{${\boldsymbol y}$}}
%\newcommand{\vyh}{\mbox{${\boldsymbol \check y}$}}
%\newcommand{\vyht}{\mbox{${\boldsymbol \hat y}$}}
%\newcommand{\vnh}{\mbox{${\boldsymbol \check n}$}}
%\newcommand{\omn}{\mbox{${\om_{_N}}$}}
%\newcommand{\pikon}{\mbox{${\frac{2\pi k}{N}}$}}



% Abrreviations
\newcommand{\ie}{\hbox{i.e.}}
\newcommand{\eg}{\hbox{e.g.}}

\def\urltilda{\kern -.15em\lower .7ex\hbox{\~{}}\kern .04em}




